DAppSCAN: Building Large-Scale Datasets for Smart Contract Weaknesses in DApp Projects

The Smart Contract Weakness Classification Registry (SWC Registry) is a widely recognized list of smart contract weaknesses specific to the Ethereum platform. Despite the SWC Registry not being updated with new entries since 2020, the sustained development of smart contract analysis tools for detecting SWC-listed weaknesses highlights their ongoing significance in the field. However, evaluating these tools has proven challenging due to the absence of a large, unbiased, real-world dataset. To address this problem, we aim to build a large-scale SWC weakness dataset from real-world DApp projects. We recruited 22 participants and spent 44 person-months analyzing 1,199 open-source audit reports from 29 security teams. In total, we identified 9,154 weaknesses and developed two distinct datasets, i.e., DAPPSCAN-SOURCE and DAPPSCAN-BYTECODE. The DAPPSCAN-SOURCE dataset comprises 39,904 Solidity files, featuring 1,618 SWC weaknesses sourced from 682 real-world DApp projects. However, the Solidity files in this dataset may not be directly compilable for further analysis. To facilitate automated analysis, we developed a tool capable of automatically identifying dependency relationships within DApp projects and completing missing public libraries. Using this tool, we created DAPPSCAN-BYTECODE dataset, which consists of 6,665 compiled smart contract with 888 SWC weaknesses. Based on DAPPSCAN-BYTECODE, we conducted an empirical study to evaluate the performance of state-of-the-art smart contract weakness detection tools. The evaluation results revealed sub-par performance for these tools in terms of both effectiveness and success detection rate, indicating that future development should prioritize real-world datasets over simplistic toy contracts.

==> attacks.tex <==
\section{SWC in Security Events}

\subsection{Motivation}
\label{sec:attack_motivation}
In section~\ref{sec:SWC}, we investigate the frequency of SWC weaknesses in real-world DApps. However, the presence of some SWC weaknesses in a contract does not mean that it will be attacked or lose Ethers. For example, the SWC-120 weakness (Weak Sources of Randomness from Chain Attributes) indicates that using block timestamp to generate a random number is not safe, as miners can control the timestamp of a block in a few seconds. It is true that malicious miners can attack contracts through this weakness; however, this kind of attack may be rare in real-world situations. Nowadays, most miners choose to join a mining pool~\cite{miners, mining_pool}, which collects a large amount of mining power. Thus, it is not easy for a single miner to mine a block on the Ethereum network with Proof-of-Work mechanism~\cite{ethereum}. Miners in the mining pool should follow some protocols and share the rewards based on their contributions. There is a low probability for these mining pools to change their strategy to attack some contracts, as misbehaving behavior could damage their reputation and lead to more losses than they earned. Furthermore, generating a random number is not easy on the blockchain. Although some blockchain oracles provide safe methods to generate random numbers, e.g., Chainlink~\cite{chainlink}, the service is usually expensive. Thus, although some developers may be aware that their contracts could be exploited by misbehaving minors, it is also hard to find a better way to generate a secure and free random numbers.

Thus, it is worth investigating whether there are real security events on Ethereum based on SWC weakness. It might be more valuable if we contribute more research efforts to analyzing the SWC weaknesses that can lead to huge financial losses. 

\subsection{Methodology}

\subsubsection{Participant Recruitment} We sent invitations to the students as we described in Section~\ref{sec:swc_recruit} and recruited 5 master's students to analyze security events. These five master's students also had good knowledge in smart contract programming but had not yet published any academic works. Thus, they also participated in the SWC training introduced in Section~\ref{sec:swc_analysis}, and the management team was also responsible for answering their questions about the SWC Registry. 

\subsubsection{Data Collection}
Two well-known security teams, i.e., SlowMist~\cite{slowmisthacked} and Rekt~\cite{rekt}, have already collected blockchain security events. Thus, we first crawled the security events reported by these two teams. By July 2022, we totally collected 148 and 149 security events from SlowMist and Rekt, respectively. To ensure the completeness of our dataset, we also collected 5,269 blockchain-related news articles from search engine.

\subsubsection{Data Analysis}
Unlike audit reports, which contain detailed descriptions of a weakness, understanding the key reasons for a security event is much more difficult. The five masters were required to search for more information about the event, e.g., the name of the exploited project, the financial loss, the exploited time, a summary of the security event, and a reference of the event. After understanding the attacks, they were required to identify whether the event was caused by an SWC weakness and a related SWC type. To ensure the correctness, each security event was checked by two masters independently. Then, they compared their results and discussed the differences. If they could not reach an agreement, the management team helped reach a final decision. 

Note that we only focused on security events on Ethereum; although we collected 5,269 news articles, most of them were not related to attacks. Moreover, there was a large amount of repeated information, as most security events were reported on by multiple platforms. All of the irrelevant and repeated information was removed during our manual analysis process. 



\begin{table}
	\caption{Security events caused by SWC Weaknesses on Ethereum} 
	\label{tab:attacks}  
	\centering
	\small
	\begin{tabular}{p{40pt} <{\centering}  | p{30pt}<{\centering} | r | r}
		\hline
		\textbf{SWC-ID} & \textbf{\#Times} & \textbf{Total Lost} & \textbf{Loss / Event}\\
		\hline
		107 & 18 & 308,720,000 & 17,151,111\\ 
		\hline 
		101 & 6 & 1,145,700,000 & 190,950,000\\ 
		\hline 
		104 & 4 & 645,200,000 & 161,300,000\\ 
		\hline 
		122 & 4 & 326,242,000 & 81,560,500 \\ 
		\hline 
		105 & 3 & 7,833,900& 2,611,300 \\ 
		\hline 
		112 & 2 & 182,211,000& 91,105,500\\
		\hline
		100 & 2 & 3,137,800 & 1,568,900\\
		\hline
		128 & 1 & 4,558,859,480& 4,558,859,480 \\
		\hline
		129 & 1 & 80,000,000  & 80,000,000  \\
		\hline
		111 & 1 & 27,600,000 & 27,600,000 \\
		\hline
		\hline
		Total & 42 & 7,285,504,180 & / \\
		\hline
	\end{tabular} \vspace{-0.4cm}
\end{table}

\subsection{Results}

After removing irrelevant and repeated information, we finally collected 281 security events on Ethereum. These events led to a financial loss of USD 73,943,943,552 in total. Among them, 42 events (14.9\%) were caused by SWC weaknesses and these led to a loss of USD 7,285,504,180. Detailed information on these security events is listed in Table~\ref{tab:attacks}. 

Only 10 kinds of SWC weakness led to 42 security events on Ethereum. \textbf{SWC-107 (Reentrancy)} had the highest frequency of leading to attacks. About 42.86\% SWC-related security events were caused by Reentrancy, with a total financial loss of USD 0.3 billion. However, neither the total financial loss nor the average loss per event (the last column in Table~\ref{tab:attacks}) was the most serious for Reentrancy attacks. Reentrancy attacks are among of the famous attacks on Ethereum. This weakness allows hackers to call the victim contract several times in a single transaction. The first Reentrancy attack, the notorious DAO attack~\cite{DAO}, happened in 2016. Although the vulnerable code example of the DAO attack has been widely publicized by blogs, books, and journals today, Reentrancy events still happen almost every year. Many new kinds of Reentrancy attack methods were born with this event. For example, the flash loan~\cite{wang2020towards} strategy has been widely used in reentrancy attacks as it can reduce the risk of the attack. Furthermore, the birth of the EIP-777 standard~\cite{ERC777} introduced a new weakness to smart contracts. Specifically, transferFrom() of EIP-777 has a callback mechanism, which may lead to a reentrancy attack if a reentrancy lock is missing. 

Although \textbf{SWC-128 (DoS with Block Gas Limit)} only led to one security event, it caused the highest financial loss. On Ethereum, the maximum gas consumption of a block is fixed. The execution of a function exceeding the maximum gas consumption of a block will lead to the denial of service. The only project exploited by SWC-128 was a game contract named Fomo3D~\cite{fomo3d}. In the Fomo3D game, users can transfer Ethers to the contract, and the latter user should pay more than the previous one. The last user when the timer runs out, is declared the winner and receives all the Ethers. The hacker used a contract to exhaust the gas in a block to raise the DoS attack when he became the last person. This attack might be regarded as a special case for the exploitation of the SWC-128 weakness, as raising this attack is not easy.  First, the hacker should be able to monitor the price function of the contract. Second, the hacker's contract can exhaust the gas in a block, which is the most important step. In this security event, the hacker set a high gas price in order to make miners execute their transactions first. However, this method is risky as a miner may discover the malicious intent and execute other transactions.

\textbf{SWC-101 (Integer Overflow and Underflow)} had the second highest attack frequency. It also had the second highest total loss per attack among all the SWC attacks. In Solidity programming, each value type has a maximum size. For example, the type \textit{uint8} can only store an 8 bit unsigned number ranging from 0 to 255. For the case of a \textit{uint8} variable 0 minus 1, the value will become 255, which is called integer underflow. Integer overflow/underflow can lead to serious security issues. The latest SWC-101 attack happened on March 20, 2022. A project named the Umbrella network had an underflow in its withdraw function, which allowed attackers to withdraw an arbitrary amount of tokens from the smart contract~\cite{swc101}. The SWC-101 weakness can be avoided by using the SafeMath library~\cite{safemath}. 

Both SWC-104 (Unchecked Call Return Value) and SWC-122 (Lack of Proper Signature Verification) led to four security events, but the financial losses caused by SWC-104 were twice those caused by SWC-122. Five kinds of SWC weakness only led to one or two security events. However, the financial losses for each event were at least USD 1.56 million, which shows the importance of detecting and removing these SWC weakness from contracts. 

For 27 kinds of SWC weaknesses we could not find any related security events. Although this finding cannot prove that contracts with these SWC weaknesses will not be attacked, it shows that more research efforts may need to be devoted to the 10 weaknesses listed in Table~\ref{tab:attacks}.


